CL$^2$GEC: A Multi-Discipline Benchmark for Continual Learning in Chinese Literature Grammatical Error Correction

The growing demand for automated writing assistance in diverse academic domains highlights the need for robust Chinese Grammatical Error Correction (CGEC) systems that can adapt across disciplines. However, existing CGEC research largely lacks dedicated benchmarks for multi-disciplinary academic writing, overlooking continual learning (CL) as a promising solution to handle domain-specific linguistic variation and prevent catastrophic forgetting. To fill this crucial gap, we introduce CL$^2$GEC, the first Continual Learning benchmark for Chinese Literature Grammatical Error Correction, designed to evaluate adaptive CGEC across multiple academic fields. Our benchmark includes 10,000 human-annotated sentences spanning 10 disciplines, each exhibiting distinct linguistic styles and error patterns. CL$^2$GEC focuses on evaluating grammatical error correction in a continual learning setting, simulating sequential exposure to diverse academic disciplines to reflect real-world editorial dynamics. We evaluate large language models under sequential tuning, parameter-efficient adaptation, and four representative CL algorithms, using both standard GEC metrics and continual learning metrics adapted to task-level variation. Experimental results reveal that regularization-based methods mitigate forgetting more effectively than replay-based or naive sequential approaches. Our benchmark provides a rigorous foundation for future research in adaptive grammatical error correction across diverse academic domains.

==> tables/qwen_scales.tex <==
\begin{table*}[htb!]
\centering
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.2}

\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{l l
                *{3}{c}  % GEC Rnd
                *{3}{c}  % GEC Sem
                *{3}{c}  % AvgPerf Rnd
                *{3}{c}  % AvgPerf Sem
                *{3}{c}  % BWT Rnd
                *{3}{c}  % BWT Sem
               }
\toprule
\multirow{2}{*}{\textbf{Model Scale}} & \multirow{2}{*}{\textbf{Strategy}}
  & \multicolumn{3}{c}{\textbf{GEC (Rnd)}} & \multicolumn{3}{c}{\textbf{GEC (Sem)}}
  & \multicolumn{3}{c}{\textbf{AvgPerf (Rnd)}} & \multicolumn{3}{c}{\textbf{AvgPerf (Sem)}}
  & \multicolumn{3}{c}{\textbf{BWT (Rnd)}}    & \multicolumn{3}{c}{\textbf{BWT (Sem)}}    \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}
\cmidrule(lr){9-11}\cmidrule(lr){12-14}
\cmidrule(lr){15-17}\cmidrule(lr){18-20}
 & 
  & P & R & F$_{0.5}$  & P & R & F$_{0.5}$
  & P & R & F$_{0.5}$  & P & R & F$_{0.5}$
  & P & R & F$_{0.5}$  & P & R & F$_{0.5}$ \\
\midrule
\multirow{4}{*}{\makecell{\textbf{Qwen2.5}\\\textbf{3B-Instruct}}}
  & SeqFT  
      & … & … & … & … & … & … 
      & … & … & … & … & … & … 
      & … & … & … & … & … & … \\
\cdashline{2-20}[1pt/1pt]
  & LoRA   
      & … & … & … & … & … & … 
      & … & … & … & … & … & … 
      & … & … & … & … & … & … \\
\cdashline{2-20}[1pt/1pt]
  & EWC    
      & … & … & … & … & … & … 
      & … & … & … & … & … & … 
      & … & … & … & … & … & … \\
\cdashline{2-20}[1pt/1pt]
  & Replay 
      & … & … & … & … & … & … 
      & … & … & … & … & … & … 
      & … & … & … & … & … & … \\
\midrule
\multirow{4}{*}{\makecell{\textbf{Qwen2.5}\\\textbf{1.5B-Instruct}}}
  & SeqFT  
      & … & … & … & … & … & … 
      & … & … & … & … & … & … 
      & … & … & … & … & … & … \\
\cdashline{2-20}[1pt/1pt]
  & LoRA   
      & … & … & … & … & … & … 
      & … & … & … & … & … & … 
      & … & … & … & … & … & … \\
\cdashline{2-20}[1pt/1pt]
  & EWC    
      & … & … & … & … & … & … 
      & … & … & … & … & … & … 
      & … & … & … & … & … & … \\
\cdashline{2-20}[1pt/1pt]
  & Replay 
      & … & … & … & … & … & … 
      & … & … & … & … & … & … 
      & … & … & … & … & … & … \\
\bottomrule
\end{tabular}
} % end resizebox
\caption{\textbf{Performance Comparison Across Qwen Model Scales on \Benchmark{}.}
We compare Qwen2.5–3B and Qwen2.5–1.5B under four strategies (SeqFT, LoRA, EWC, Replay with 5\% buffer) for Random vs.\ Semantic task orders.  
Metrics: GEC (P / R / F$_{0.5}$), Avg.\ Performance (P / R / F$_{0.5}$), Backward Transfer (P / R / F$_{0.5}$).}
\label{tab:qwen_scale_results}
\end{table*}



% \begin{table*}[htb!]
% \centering
% \caption{\textbf{Performance Comparison Across Qwen Model Scales on \Benchmark{}.}
% We compare Qwen2.5–3B and Qwen2.5–1.5B under four strategies (SeqFT, LoRA, EWC, Replay with 5\% buffer) for Random vs.\ Semantic task orders. Metrics reported: average GEC (P, R, $F_{0.5}$), Avg.\ Performance (P, R, $F_{0.5}$) and Backward Transfer (P, R, $F_{0.5}$).}
% \label{tab:qwen_scale_results}
% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1.1}

% \begin{tabular}{lll *{3}{c} *{3}{c} *{3}{c}}
% \toprule
% \textbf{Model Scale} & \textbf{Strategy} & \textbf{Order}
%   & \multicolumn{3}{c}{\textbf{GEC}}
%   & \multicolumn{3}{c}{\textbf{AvgPerf}}
%   & \multicolumn{3}{c}{\textbf{BWT}} \\
% \cmidrule(lr){4-6} \cmidrule(lr){7-9} \cmidrule(lr){10-12}
%  & & 
%   & P & R & F$_{0.5}$
%   & P & R & F$_{0.5}$
%   & P & R & F$_{0.5}$ \\
% \midrule
% \multirow{8}{*}{\makecell{\textbf{Qwen2.5}\\\textbf{3B-Instruct}}}
%   %--- SeqFT
%   & \multirow{2}{*}{SeqFT}
%       & Random   & … & … & … & … & … & … & … & … & … \\
%   &
%       & Semantic & … & … & … & … & … & … & … & … & … \\
%   %--- LoRA
% \cdashline{3-12}[1pt/1pt]
%   & \multirow{2}{*}{LoRA}
%       & Random   & … & … & … & … & … & … & … & … & … \\
%   &
%       & Semantic & … & … & … & … & … & … & … & … & … \\
%   %--- EWC
% \cdashline{3-12}[1pt/1pt]
%   & \multirow{2}{*}{EWC}
%       & Random   & … & … & … & … & … & … & … & … & … \\
%   &
%       & Semantic & … & … & … & … & … & … & … & … & … \\
%   %--- Replay
% \cdashline{3-12}[1pt/1pt]
%   & \multirow{2}{*}{Replay}
%       & Random   & … & … & … & … & … & … & … & … & … \\
%   &
%       & Semantic & … & … & … & … & … & … & … & … & … \\
% \midrule
% \multirow{8}{*}{\makecell{\textbf{Qwen2.5}\\\textbf{1.5B-Instruct}}}
%   %--- SeqFT
%   & \multirow{2}{*}{SeqFT}
%       & Random   & … & … & … & … & … & … & … & … & … \\
%   &
%       & Semantic & … & … & … & … & … & … & … & … & … \\
%   %--- LoRA
% \cdashline{3-12}[1pt/1pt]
%   & \multirow{2}{*}{LoRA}
%       & Random   & … & … & … & … & … & … & … & … & … \\
%   &
%       & Semantic & … & … & … & … & … & … & … & … & … \\
%   %--- EWC
% \cdashline{3-12}[1pt/1pt]
%   & \multirow{2}{*}{EWC}
%       & Random   & … & … & … & … & … & … & … & … & … \\
%   &
%       & Semantic & … & … & … & … & … & … & … & … & … \\
%   %--- Replay
% \cdashline{3-12}[1pt/1pt]
%   & \multirow{2}{*}{Replay}
%       & Random   & … & … & … & … & … & … & … & … & … \\
%   &
%       & Semantic & … & … & … & … & … & … & … & … & … \\
% \bottomrule
% \end{tabular}

% \end{table*}

